A Vision for Online Verification-Validation

Today's programmers face a false choice between creating software that is extensible and software that is correct. Specifically, dynamic languages permit software that is richly extensible (via dynamic code loading, dynamic object extension, and various forms of reflection), and today's programmers exploit this flexibility to "bring their own language features" to enrich extensible languages (e.g., by using common JavaScript libraries). Meanwhile, such library-based language extensions generally lack enforcement of their abstractions, leading to programming errors that are complex to avoid and predict. To offer verification for this extensible world, we propose online verification-validation (OVV), which consists of language and VM design that enables a "phaseless" approach to program analysis, in contrast to the standard static-dynamic phase distinction. Phaseless analysis freely interposes abstract interpretation with concrete execution, allowing analyses to use dynamic (concrete) information to prove universal (abstract) properties about future execution. In this paper, we present a conceptual overview of OVV through a motivating example program that uses a hypothetical database library. We present a generic semantics for OVV, and an extension to this semantics that offers a simple gradual type system for the database library primitives. The result of instantiating this gradual type system in an OVV setting is a checker that can progressively type successive continuations of the program until a continuation is fully verified. To evaluate the proposed vision of OVV for this example, we implement the VM semantics (in Rust), and show that this design permits progressive typing in this manner.

==> Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = paper

PAPERS = $(BASE)
BIBS = $(wildcard *.orig.bib)
SHORT_BIBS= $(BIBS:%.orig.bib=%.short.bib)
OTTFILE = vmf-def.ott
MNG = $(wildcard *.mng.tex)

DEPS = $(SHORT_BIBS) $(OTTFILE:%.ott=%.tex) $(MNG:%.mng.tex=%.tex)
SRCS = $(wildcard *.tex) $(wildcard *.sty) $(DEPS)

.PHONY: html pdf all

all: pdf
shortbibs: $(SHORT_BIBS)
pdf: $(PAPERS:%=%.pdf)
html: $(PAPERS:%=%/index.html)

$(PAPERS:%=%.pdf): $(SRCS)

cleandeps:
	rm -f $(DEPS)
clean: cleandeps
	latexmk -c
cleanall: cleandeps
	latexmk -C

# Generate TR TeX
%.tr.tex: %.tex
	sed 's/\\TRfalse/\\TRtrue/' $< >$@

# Generate Posting Version TeX
%.post.tex: %.tex
	sed 's/\\Postingfalse/\\Postingtrue/' $< >$@

# Generate PDF
%.pdf: %.tex
	latexmk -pdf -use-make $<

# Generate short bib
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@

%.txt: %.tex
	cat $< | detex | sed 's/---/--/g' > $@

%-def.tex: %-def.ott
	ott $< -tex_wrap false -o $@

%.tex: %.mng.tex
	ott $(OTTFILE) -tex_filter $< $@


==> mk <==
#!/bin/sh
export PATH=$PATH:/Users/hammer/Downloads/ott_distro_0.25/bin/
ottfile=vmf-def.ott
#ott $ottfile -tex_wrap true -o vmf-def-full.tex
#pdflatex vmf-def-full
ott $ottfile -tex_wrap false -o vmf-def.tex \
    && ott $ottfile -tex_filter sec-vmf.mng.tex sec-vmf.tex \
    && pdflatex paper



==> mk_ <==
#!/bin/sh
ottfile=vmf-def.ott
#ott $ottfile -tex_wrap true -o vmf-def-full.tex
#pdflatex vmf-def-full
ott $ottfile -tex_wrap false -o vmf-def.tex \
    && ott $ottfile -tex_filter sec-vmf.mng.tex sec-vmf.tex \
    && pdflatex main-vmf


==> sec-vmf.mng.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{OVV Machine Semantics}
\label{sec:vm-semantics}
\label{sec:vmf}

We present \lambdaVMF, an abstract machine semantics for libraries
and programs that employ OVV.  In \secref{typing}, we instantiate
this OVV framework with a gradual type system for checking programs
that compute with simple databases.

\paragraph{Program Syntax.}
%
\figref{syntax} gives the syntax for \lambdaVMF programs.
%
To streamline the definition of analyses and dynamic interpretation,
\lambdaVMF syntactically separates program structure into expressions~$[[e]]$
and values~$[[v]]$.
%
Further, to permit a meta-layer, extension-defined analysis to
annotate \lambdaVMF programs (as illustrated in \secref{typing}), the
recursive syntax of expressions and values consists of annotated
pre-expressions~$[[pe]]$ and annotated pre-values~$[[pv]]$,
respectively.
%
The operational semantics of \lambdaVMF programs, defined below, does
not directly depend on these annotations.  However, an extension
may use its annotations to prove properties that verify sound online
program transformations.  In these cases, the annotations can
indirectly impact program behavior, i.e., by aiding a meta-level
program transformation.

Pre-values consist of open and closed thunks, which represent suspended
expressions, including all higher-order data~($[[othunk e]]$ and
$[[thunk env e]]$); closed thunks employ a closing
environment~$[[env]]$ that maps the free variables of~$[[e]]$ to
(closed) values.
%
Base types consist of numbers~($[[num n]]$), strings~($[[str s]]$),
boolean bits~($[[bool b]]$) and reference cells~($[[loc l]]$).
%
Dictionaries map values to values~($[[dict delta]]$), modeling a row
of a database, or a record, where the typical notion of a field name
is generalized to any value in \lambdaVMF.

Pre-expressions consist of forcing a suspended expression~($[[force v]]$),
function abstraction~($[[lam x.e]]$), function application~($[[e
    v]]$), let-binding a returned value ($[[let x = e1 in e2]]$),
returning a value~($[[ret v]]$), allocating, mutating and accessing
mutable storage ($[[ref v]]$, $[[set v1 v2]]$, $[[get v]]$,
respectively), updating the field of a record ($[[ext v1 v2 v3]]$),
projecting the field of a record ($[[proj oa v1 v2]]$).

Finally, \lambdaVMF includes special forms for ascribing a
sub-expression with a manual annotation ($[[e ?: ae]]$),
%
and reflectively inspecting (and transforming) the current continuation via
\lstinline{reflect/cc} as core primitive, $[[rcc me e]]$.
%
Notably, execution pauses \emph{before} executing the local
continuation~$[[e]]$, and a common idiom consists of using a manual
ascription there, to be discharged via the use of $\ottkw{rcc}$.

As explained below, using $\ottkw{rcc}$ to prove and discharge
ascriptions is actually necessary in \lambdaVMF, since they have no
other form of dynamic semantics. \TODO{I think we should expand this discussion. This is the interesting part. -Evan}
%
For this purpose, the meta-level program $[[me]]$ transforms the
program state before its continuation resumes.
%
We do not model the model-level programming language here; our current
implementation uses Rust.

\begin{figure}
\small
\begin{jgrammar}
  Value    & $[[v]]$& $\bnfas$& $[[pv @: av]]$ & Annotated pre-value
  \\
  Pre-Val. & $[[pv]]$
  &$\bnfas$&        $[[othunk e]]$    & Open thunk
  \\ &&& $\bnfaltbrk [[thunk env e]]$ & Closed thunk
  \\ &&& $\bnfaltbrk [[dict delta]]$  & Dictionary
  \\ &&& $\bnfaltbrk [[num n]]$ & Number
  \\ &&& $\bnfaltbrk [[str s]]$ & String
  \\ &&& $\bnfaltbrk [[bool b]]$ & Boolean
  \\ &&& $\bnfaltbrk [[loc l]]$ & Store location
  \\ &&& $\bnfaltbrk [[()]]$    & Unit value
  \\ &&& $\bnfaltbrk [[x]]$     & Value variable
  \\
  Dict. & $[[ delta ]]$
  &$\bnfas$& $[[ emp ]]~|~[[ delta , v1 => v2 ]]$ & Dictionaries of values
  \\[2mm]
  Expr.     & $[[e]]$& $\bnfas$& $[[pe @: ae]]$ & Annotated pre-expression
  \\
  Pre-Expr. & $[[pe]]$ & $\bnfas$ & $[[force v]]$ & Unsuspend (force) thunk
  \\ &&& $\bnfaltbrk [[lam x. e]]$ & Function abstraction
  \\ &&& $\bnfaltbrk [[ e v ]]$ & Function application
  \\ &&& $\bnfaltbrk [[let x = e1 in e2]]$ & Bind computed value
  \\ &&& $\bnfaltbrk [[ret v]]$ & Produce a value
  \\ &&& $\bnfaltbrk [[ref v]]$ & Allocate store reference
  \\ &&& $\bnfaltbrk [[set v1 v2]]$ & Store mutation
  \\ &&& $\bnfaltbrk [[get v]]$ & Store projection
  \\ &&& $\bnfaltbrk [[ext v1 v2 v3]]$ & Dictionary extension
  \\ &&& $\bnfaltbrk [[proj oa v1 v2]]$ & Dictionary projection
  \\ &&& $\bnfaltbrk [[e ?: ae]]$ & Annotation ascription
  \\ &&& $\bnfaltbrk [[rcc me e]]$ & Reflect current continuation
  \\[2px]
  Annot.
    & $[[oa]]$ & $\bnfas$ & $[[ ? ]]~|~[[ ! ]]$ & Uncertain vs. certain
  \\
    & $[[av]]$ & $\bnfas$ & $\cdots$ & Value annotation
  \\
    & $[[ae]]$ & $\bnfas$ & $\cdots$ & Expression annotation
 \\[2px]
 Meta Expr.
   & $[[me]]$ & $\bnfas$ & $\cdots$ & Meta-level programs
\end{jgrammar}
\caption{Syntax of \lambdaVMF Programs}
\label{fig:syntax}
\end{figure}

\begin{figure}
  \small
  \begin{jgrammar}
    State
    & $[[state]]$ & $\bnfas$ & $[[ <store; stack; env; pe> ]]$ &
    \\
    Store
    & $[[store]]$ & $\bnfas$ & $[[ emp ]]~|~[[ store, l => v ]]$ & Maps locations to values
    \\
    Stack
    & $[[stack]]$ & $\bnfas$ & $[[ halt ]]$ & Empty stack
    \\
    &&& $\bnfaltbrk [[ stack :::: (env, x.e)  ]]$ & Waiting for return
    \\
    &&& $\bnfaltbrk [[ stack :::: v  ]]$ & Fun. application argument
    \\
    Environment
    & $[[env]]$   & $\bnfas$ & $[[ emp ]]~|~[[ env,   x => v ]]$ & Maps variables to values
  \end{jgrammar}
  \caption{VM State: The store, stack and environment.}
  \label{fig:state}
\end{figure}

\paragraph{VM State syntax.}
\figref{state} defines the global state of the \lambdaVMF program: It
consists of a store, mapping locations to mutable
values~($[[store]]$); a stack of evaluation context frames
($[[stack]]$), an environment mapping variables to values~($[[env]]$),
and a pre-expression~$[[pe]]$ that gives the current local
continuation.
%
Non-empty stacks give evaluation contexts for $\ottkw{let}$
bodies~($[[stack :::: (env, x.e)]]$) and function
application~($[[stack :::: v]]$).

\paragraph{Dynamics of \lambdaVMF Programs.}

\begin{figure*}
\small
\judgbox{[[ state --> state' ]]}{
  \lambdaVMF state~$[[state]]$ steps to state~$[[state']]$.
}
\[
\begin{array}{@{\hspace{-10mm}}rlclcl}
[[ <store; stack; env | let x = (pe1@:__) in e2> --|--> <store; stack :::: (env, x. e2); env; pe1> ]]
\\
[[ <store; stack; env | (pe@:__) v> --|--> <store; stack :::: lookup env v; env; pe> ]]
\\
[[ <store; stack :::: (env, x.(pe@:__)); env' | ret v> --|--> <store; stack; env, x => lookup env v; pe> ]]
\\
[[ <store; stack :::: v; env | lam x.(pe@:__)> --|--> <store; stack; env, x => v; pe> ]]
\\
[[ <store; stack; env | force v> --|--> <store; stack; env'; pe> ]]
& \textrm{when} & [[ env v ~> (thunk env' (pe@:__) @: __) ]]
\\
[[ <store; stack; env | ref v> --|--> <store, l => v; stack; env; ret (loc l @: ?)> ]]
& \textrm{when} & [[ l notin store ]]
\\
[[ <store; stack; env | set v1 v2> --|--> <store, l => lookup env v2; stack; env; ret (() @: ?)> ]]
& \textrm{when} & [[ env v1 ~> (loc l @: __) ]]
\\
[[ <store, l=>v2; stack; env | get v1> --|--> <store, l=>v2; stack; env; ret v2> ]]
& \textrm{when} & [[ env v1 ~> (loc l @: __) ]]
\\
[[ <store; stack; env | ext v1 v2 v3> --|--> <store; stack; env; ret (dict (delta, lookup env v2=> lookup env v3)@:?)> ]]
& \textrm{when} & [[ env v1 ~> (dict delta @: __) ]]
\\
[[ <store; stack; env | proj ! v1 v2> --|--> <store; stack; env; ret v3> ]]
& \textrm{when} & [[ env v1 ~> (dict (delta, lookup env v2 => v3) @: __) ]]
\\[2mm]
[[ <store; stack; env | proj ? v1 v2 > ]] & \multicolumn{2}{l}{\textit{no stepping rule}}
\\
[[ <store; stack; env | e ?: ae > ]] & \multicolumn{2}{l}{\textit{no stepping rule}}
\\[2mm]
[[ <store; stack; env | rcc me (pe@:__)> --|--> state' ]]
& \textrm{when} & [[meta me <store; stack; env; pe> ~~> state']]
\end{array}
\]
\caption{Small-step, abstract machine semantics of \lambdaVMF}
\label{fig:step}
\end{figure*}

\figref{step} defines a small-step operational semantics over \lambdaVMF states.
%
The rules for $\ottkw{let}$ and function application each push the
stack with a frame that is eliminated by the rules for $\ottkw{ret}$
and function abstraction, respectively.
%
In both cases, eliminating the frame consists of binding a value to a
variable, and continuing the program.
%
Forcing a thunk consists of unpacking its environment and expression,
and continuing execution with them.
%
Rules for allocating, mutating and accessing a reference cell in the
store are each standard.
%
Dictionary extension adds a field to a (possibly empty) dictionary;
and dictionary projection selects a given field's associated value,
returning it.

What makes \lambdaVMF particularly interesting is that
there are no stepping rules for $[[?]]$-mode field projection
or for ascription.
%
To avoid getting stuck at these operations, these operations should be
either verified progressively or validated, perhaps immediately before
executing, when all relevant information is available.
%
To do so, the program uses $[[rcc me e]]$, which runs the meta-level
program $[[me]]$ on a reflected version of the current VM state: the
rule constructs the current continuation, reflects this program state
into a data structure, runs the meta-level term~$[[me]]$, and then
injects the resulting program state into a transformed
continuation~$[[state']]$.
%
In OVV, this step sometimes verifies and validates operations before
the program attempts to execute them, transforming the program to
remove or modify them.
%
In contrast to traditional phasic static verification or dynamic validation (cf.
\figref{phasic-grid}), this step does not need to be either eagerly before the
entire execution or lazily just before the potentially faulting operation. By
choosing the placement of $\ottkw{rcc}$, the program can choose how eager or
lazy the checking should be anywhere between these two extremes.
%
We give a detailed example below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Bidirectional Gradual Typing}
\section{Gradual Typing for Simple Databases}
\label{sec:typing}

In this section we present a gradual type system for \lambdaVMF and
\textsf{libDb}, an extension that permits us to express the motivating
example from \figref{full-example-code}.
%
We tour the type system and illustrate how OVV progressively types and
validates the operations in this example.

\begin{figure}
  \small
  \begin{jgrammar}
  & $e$
    &$\bnfas$& $\cdots$ & Existing forms (\Figref{syntax})
    \\ &&& $\bnfaltbrk [[ openDb oa v ]]$ & Open database by file path
    \\ &&& $\bnfaltbrk [[ filterDb oa v1 v2 ]]$ & Filter DB by predicate
    \\ &&& $\bnfaltbrk [[ joinDb oa v1 v2 v3 v4 ]]$ & Join DBs using keys' value
\end{jgrammar}
\caption{Database Library Forms}
\label{fig:db-syntax}
\end{figure}

\paragraph{Syntax for \textsf{libDb}.}
\figref{db-syntax} extends the syntax from \figref{syntax} with the three
operations implemented by \libDb, for opening databases, filtering
them with a predicate, and joining them using named fields.
%
Each operation is parameterized by one or more argument values, and an
operation annotation $[[oa]]$ that determines how to type operation.
%
As with record field projection, this annotation determines whether
the operation's pre-conditions for success have been fully verified
via OVV.
%
The gradual type system for \libDb presented here uses different rules
for certain ($[[!]]$) versus uncertain ($[[?]]$) reasoning modes.

\paragraph{Types for \lambdaVMF and \textsf{libDb}.}
\figref{types} instantiates the \lambdaVMF framework for a gradual
type system.  This system has (bidirectional, algorithmic) rules to
reason about \lambdaVMF code as well as the \libDb extension.
%
Value types consist of types for thunked computations~($[[U C]]$)
%
\footnote{ We follow conventions from the literature on
  call-by-push-value (CBPV) in our type syntax for thunked and
  value-returning computations, which uses special letters \textbf{U}
  and \textbf{F}, respectively~\cite{Levy99subsuming,levy2003call}.
%
},
dictionaries ($[[Dict Delta]]$, where $[[Delta]]$ maps field values to
field types), numbers~($[[Num]]$), strings~($[[Str]]$), booleans~($[[Bool]]$), reference
cells~($[[Ref A]]$), unit~($[[1]]$), unknown~($[[?]]$) and
databases ($[[Db A]]$).
%
Computation types consist of the arrow type for functions~($[[A ->
    C]]$) and value types for value-producing computations~($[[F
    A]]$).

\begin{figure}
\small
\begin{jgrammar}
  Annotations
    & $[[av]]$ & $\bnfas$ & $[[A]]$ & Value annotation
  \\
    & $[[ae]]$ & $\bnfas$ & $[[C]]$ & Expression annotation
  \\
  Value Types  & $[[A]], [[B]]$& $\bnfas$&
  $ [[U C]]$& Thunked computation
  \\ &&& $\bnfaltbrk [[Dict Delta]]$& Dictionary
  \\ &&& $\bnfaltbrk [[Num]]$& Number
  \\ &&& $\bnfaltbrk [[Str]]$& String
  \\ &&& $\bnfaltbrk [[Bool]]$& Boolean
  \\ &&& $\bnfaltbrk [[Ref A]]$& Reference cell
  \\ &&& $\bnfaltbrk [[1]]$& Unit
  \\ &&& $\bnfaltbrk [[?]]$& Unknown value type
  \\ &&& $\bnfaltbrk [[Db A]]$& Database; multiset of $[[A]]$s
  \\[2mm]
  Dictionary & $[[Delta]]$ & $\bnfas$ & \multicolumn{2}{l}{$[[emp]]~|~[[Delta, v => A]]$~~~\textrm{Maps values to types}}
  \\[2mm]
  Computation & $[[C]], [[D]]$ & $\bnfas$&
  %\\ &&&
  $[[A -> C]]$ & Function abstraction
  \\
  Types
  &&& $\bnfaltbrk [[F A]]$ & Value production
\end{jgrammar}
\caption{Type Syntax: Annotations for Values and Expressions}
\label{fig:types}
\end{figure}


\begin{figure}
\small
%\begin{tabular}{c|c}
%\begin{minipage}{1.6in}
\judgbox{[[ state ok ]]}{
  State~$[[state]]$ is well-typed.
}
\begin{mathpar}
\Infer{state}
{
[[ ctxify store      |- env => Ctx ]]
\\
[[ ctxify store, Ctx |- pe => C    ]]
\\
[[ ctxify store      |- stack <= C ]]
}
{
[[ <store; stack; env; pe> ok ]]
}
\end{mathpar}
%\end{minipage}
%&
%\begin{minipage}{5.45in}
\judgbox{[[ Ctx |- stack <= C ]]}{
  Under~$[[Ctx]]$,
  stack $[[stack]]$
  eliminates a computation of type~$[[C]]$.
}
\begin{mathpar}
\Infer{k-emp}
{ }
{[[ Ctx |- halt <= C ]]}
\and
\Infer{k-let}
{
[[ Ctx1 |- env => Ctx2 ]]
\\\\
[[ Ctx2, x:A |- e => C ]]
\\\\
[[ Ctx1 |- stack <= C ]]
}
{[[ Ctx1 |- stack :::: (env, x.e) <= F A ]]}
\and
\Infer{k-app}
{
[[ Ctx |- v <= A ]]
\\\\
[[ Ctx |- stack <= C ]]
}
{[[ Ctx |- stack :::: v <= A -> C ]]}
\end{mathpar}
%\end{minipage}
%\end{tabular}
\caption{Stack typing and State typing}
\label{fig:stack-state-typing}
\end{figure}

\paragraph{Typing \lambdaVMF program states.}

\figref{stack-state-typing} lists typing judgement forms for
\lambdaVMF program states and for stacks.
%
To type a program state, we assume that the stored values are
annotated, and we use these annotations as a store typing, written
$[[ctxify store]]$, which maps reference locations to values types.
%
To type a program state, we assume this store typing~$[[ctxify
    store]]$ and attempt to verify the the other VM machinery,
consisting of the current environment~$[[env]]$, program
term~$[[pe]]$, and stack~$[[stack]]$.
%
Three judgements compute type properties for these components:
%
Assuming a store typing $[[Ctx]]$, the judgement $[[Ctx |- env =>
    Ctx']]$ computes from an environment (mapping variables to
values), a typing context~$[[Ctx']]$ (mapping variables to types).
%
Assuming a typing context $[[Ctx]]$, the judgement $[[Ctx |- e => C]]$
computes a type from a term $e$.
%
Assuming a typing context $[[Ctx]]$ and computation type~$C$ for a
terminal computation, the judgement $[[Ctx |- stack <= C]]$ checks that
the stack~$[[stack]]$ either correctly continues execution or halts.

The remainder of the figure gives three rules for type-checking the
stack.
%
First, \textrm{k-emp} says that halting stacks are always permitted.
%
Next, \textrm{k-let} and \textrm{k-app} handle the recursive cases of
the stack, where the topmost frame can be viewed as eliminating the
terminal computation type, call it~$[[D]]$.
%
In the case of \textrm{k-let}, we have that~$[[D]]$ is~$[[F A]]$,
which types the terminal computation that returns a value of
type~$[[A]]$; we check that the top of the stack holds the body of the
let, which can use the let-bound variable (of type~$[[A]]$), for which
we can synthesize another computation type~$[[C]]$ that checks against
the rest of the stack.
%
In the case of \textrm{k-app}, we have that $[[D]]$ is~$[[A -> C]]$,
the type of a function abstraction; we check that the top of the stack
is an argument value of type~$[[A]]$, and the rest of the stack checks
against the type of the abstraction's body, $[[C]]$.

\paragraph{Transforming \lambdaVMF program states.}
\JEDI{Instead of merely checking them, we transform program states}
Though the gradual type system defined here is stated
propositionally, it constitutes an algorithm, and we demonstrate this
fact by implementing these relational definitions as a (mutually)
recursive total functions.
%
However, instead of merely returning \texttt{true} or \texttt{false}
to indicate the success or failure of the relation to hold, in the
case of \texttt{true}, we also construct an annotated term, possibly
with transformations (e.g., changing operation annotations from
uncertain~$[[?]]$ to certain~$[[!]]$).

For instance, we implement the type relation for program states as a
total function from program states to (optional) program states with
annotations; and when the algorithm fails, it returns \texttt{None}:
%\begin{lstlisting}
%  xform_state : State -> Option<State>
%\end{lstlisting}
Furthermore, this algorithm plays the role of~$[[me]]$ in
\textsf{libDb}'s use of~$[[rcc me e]]$.

The ability to phrase the typing relations as functional algorithms
stems the fact that the rules treat certain positions of their
(bidirectional) relations consistently as inputs and outputs, and that
outputs are determined functionally from inputs.
%
As an example, \figref{chkCont} gives the algorithmic version of the
stack-checking relation~$[[Ctx |- stack <= C]]$, which resembles an
ordinary function in ML.
%
The remainder of the rules transform in a similar manner, so that
checking relations produce an optional, annotated term structure,
while synthesizing relations produce an optional pair of annotated
term structure and synthesized type.
%
When these functions produce \code{None}, the corresponding typing
relation is not derivable.
%
The dynamic semantics of \lambdaVMF do not permit execution to
continue when this occurs.

%% %
%% When the algorithm fails, the type system is signaling to the VM
%% runtime system that the program contains a potential inconsistency in
%% future execution, and the VM either halts preemptively, or defers to
%% other error handling protocols.\marginnote{MH: What are they?}


\begin{figure}
\small

%\end{figure}
%\begin{figure}

%\begin{tabular}{c|c}
%\begin{minipage}{3.5in}
\judgbox{[[ Ctx |- e <= C ]]}{ Under $[[Ctx]]$, expression $[[e]]$ checks against type~$[[C]]$. }
\begin{mathpar}
\Infer{sub}
{[[Ctx |- e => C ]]
  \\\\
  [[C <consis> D]]}
{[[Ctx |- e <= D ]]}
\and
\Infer{lam}
{[[Ctx, x : A |- e       <=      C]]}
{[[Ctx        |- lam x.e <= A -> C]] }
\end{mathpar}
%\end{minipage}
%&
%\begin{minipage}{3.5in}
\judgbox{[[ Ctx |- e => C ]]}{ Under $[[Ctx]]$, expression $[[e]]$ synthesizes type~$[[C]]$. }
%\end{minipage}
%\end{tabular}
\begin{mathpar}
\Infer{annot}
{[[Ctx |- e <=  C]]}
{[[Ctx |- e ?: C => C ]]}
\and
\Infer{app}
{[[Ctx |- e => A -> C]]
\\\\
[[Ctx |- v <= A]]
}
{[[Ctx |- e v => C]]}
\and
\Infer{p?}
{[[Ctx |- v1 => ?]]
\\\\
[[Ctx |- v2 => B]]
}
{[[Ctx |- proj ? v1 v2 => F ?]] }
\and
\Infer{p!}
{[[Ctx |- v1 => Dict (Delta, v2 => A)]]
\\\\
[[Ctx |- v2 => B]]
}
{[[Ctx |- proj ! v1 v2 => F A]] }
\and
\Infer{openDb?}
{[[Ctx |- v => Str]]}
{[[Ctx |- openDb ? v => F (Db ?)]]}
\and
\Infer{filterDb?}
{[[Ctx |- v1 => Db ?]]
\\\\
[[Ctx |- v2 <= U(? -> F Bool)]]
}
{[[Ctx |- filterDb ? v1 v2 => F (Db ?)]]}
\and
\Infer{filterDb!}
{[[Ctx |- v1 => Db A]] \\ [[? notin A]]
\\\\
[[Ctx |- v2 <= U(A -> F Bool)]]
}
{[[Ctx |- filterDb ! v1 v2 => F (Db A)]]}
\and
\Infer{joinDb?}
{[[Ctx |- v1 => Db ?]]
\\
[[Ctx |- v2 => B2]]
\\\\
[[Ctx |- v3 => Db ?]]
\\
[[Ctx |- v4 => B4]]
}
{[[Ctx |- joinDb ? v1 v2 v3 v4 => F (Db ?)]]}
\and
\Infer{joinDb!}
{
[[Delta = Delta1, v2 => A, Delta3, v4 => A]]
\\\\
[[Ctx |- v1 => Db (Dict (Delta1, v2 => A))]]
\\
[[Ctx |- v2 => B2]]
\\\\
[[Ctx |- v3 => Db (Dict (Delta3, v4 => A))]]
\\
[[Ctx |- v4 => B4]]
}
{[[Ctx |- joinDb ! v1 v2 v3 v4 : F (Db (Dict Delta))]]}
\end{mathpar}
\caption{Selected typing rules for computation typing (checking and synthesis).}
\label{fig:type-terms}

\vspace*{5mm}

%\subfloat[Progress typing: Uncertainty vs Certainty over execution time (vertical).]
%{
\begin{center}
\begin{tabular}{|l|cccc||c|}
\multicolumn{6}{c}{\textbf{Typing} (horizontal) across \textbf{Execution} (vertical). }
\\
\hline
       & Line 1      & Line 2       & Line 3        &  Line 4  & $\cdots$
\\
       & openDb      & filterDb     & openDb        & joinDb   & ---
\\
\hline
1: openDb & $[[?]]$ & $[[?]]$ & $[[?]]$ & $[[?]]$      & $[[?]]$
\\
\hdashline
2: filterDb & ---     & $[[!]]$ & $[[?]]$ & $[[?]]$      & $[[!]]$ / $[[?]]$
\\
3: openDb & ---     & ---     & $[[?]]$ & $[[?]]$      & $[[!]]$ / $[[?]]$
\\
\hdashline
4: joinDb & ---     & ---     & ---     & $[[!]]$      & $[[!]]$
\\
\hline
\end{tabular}
\end{center}
%}
\caption{
  Progressive typing for \figref{full-example-code}:
  As execution progresses (vertically) over Lines 1 and 3, the
  continuation's typing becomes more certain: After Line 1
  executes, Line 2 types in the certain modality ($[[!]]$) instead of
  the uncertain modality ($[[?]]$); similarly,
  after Line 3, Lines 4 onward type using the certain modality.
  (The dashed horizontal lines indicate these progressions).
}
\label{fig:time2d-typing}

\end{figure}

\paragraph{Typing core \lambdaVMF terms bidirectionally.}
For simplicity, we use a bidirectional type system to encode the
gradual type systems of the \lambdaVMF core calculus and its
\textsf{libDb} extension.
%
\figref{type-terms} defines type checking (above) and synthesis
(below) for program terms.
%
For space reasons, we elide some synthesis cases, as well as the
checking and synthesis judgements for value forms; the rules shown
give a representative flavor for the complete definition.

The analytical (checking) judgement form $[[Ctx |- e <= C]]$ can be
read as, ``Under typing context $[[Ctx]]$, term $[[e]]$ checks against
computation type $[[C]]$.''  Specifically, the type~$[[C]]$ is given
as an input to the checking judgement, when viewed as an algorithm.
%
The synthesizing judgement form $[[Ctx |- e => C]]$ can be read as,
``the typing context $[[Ctx]]$ and term $[[e]]$ \emph{synthesize} the
computation type $[[C]]$.'' Specifically, the algorithm
\emph{computes} the type~$[[C]]$, when given $[[Ctx]]$ and $[[e]]$.
%
For the core forms of \lambdaVMF, the bidirectional rules for values
and computations follow the usual patterns found in bidirectional type
systems~\cite{ChlipalaPH05,DunfieldK16}.
%
We show several standard-looking rules, \textrm{sub}, \textrm{lam},
\textrm{app} and \textrm{annot}.
%
In particular, the annotation form of \lambdaVMF, $[[e ?: ae]]$, which
asserts the annotation $[[ae]]$ correctly describes the program
$[[e]]$, plays the role of type ascription in the bidirectional rules;
the \textrm{annot} rule says that terms are checked against their type
annotations, and these annotated terms synthesize the annotation type.
%
Because it has no dynamic semantics, \lambdaVMF uses OVV to prove and
discharge this form earlier by rewriting it to $[[e]]$ sometime before
evaluation; if this rewrite fails, then the program terminates (by
failing) early, as a result of OVV failing, not execution.

As is customary in bidirectional systems, type annotations mediate
between synthesizing and checking.  This provides one the ability to
place checking-only terms (such as lambda abstractions) in positions
that require the sub-term synthesize a type (such as the abstraction
position of an application).  See typing rules \textrm{lam} and
\textrm{app}, respectively, to see the details; both are standard.
%
Finally, as is customary, type \emph{subsumption} allows less specific
types to check against terms that synthesize more specific types.
%
Rule \textrm{sub} uses a definition of type \emph{consistency}
(written $[[C <consis> D]]$), which behaves like type equality, modulo
the uncertain type~$[[?]]$, which is consistent with all other types.
%
This notion of consistency is standard in some gradual typing
literature~\cite{siek+2006:gradual-typing}.

\paragraph{Gradual typing for dictionary projection.}
%
The typing rules for uncertain and certain projection differ in what
is known about the record and field values, and illustrate a form of
gradual typing.
%
In the uncertain case, rule~\textrm{p?} synthesizes return
type~$[[?]]$, since nothing is known about the dictionary of values
being projected.
%
By contrast, in the certain case, the dictionary type is known to
rule~\textrm{p!}, and this dictionary maps the given field value to a
corresponding field type.
%
In this case, the soundness of the type system means that the
projection must succeed in all possible future program states, and
moreover, that the projected value has the given type.

\paragraph{Typing the \textsf{libDb} operations.}
%
The rule~\textrm{openDb?} is uncertain and has no certain counterpart:
The type of the database is not known until after the operation
completes, just before execution resumes with its continuation; before
then, the database could hold any type, so the rule types the returned
database as~$[[Db ?]]$.

Following similar reasoning, since filtering and joining databases
occur \emph{after} a database is loaded, it is possible to type these
operations in both uncertain and certain modes.
%
The rule~\textrm{filterDb?} says that filtering a database of
uncertain values leads to another database of values with an uncertain
type; since it merely assumes the type of the database is~$[[?]]$, it
does not prove that the predicate will not ``go wrong'', e.g., by
projecting the wrong field from its argument.
%
By contrast, the rule~\textrm{filterDb!} says that filtering a
database of known type using a predicate that checks against this type
leads to a database with the same known type; in this case, the
soundness of the type system means that the predicate must always
succeed.

Similarly, the rules for \textrm{joinDb?} and \textrm{joinDb!} follow
the pattern set above: the uncertain rule assumes nothing about the
argument values, beyond the arguments actually consisting of
databases.  The certain rule assumes that the database arguments'
types are fully known, that the chosen field values are mapped in
these types, and that the chosen fields share a common type (we want
to compare values of this field for equality to perform the join).

\paragraph{Gradual Typing, Progressively via OVV.}
%
\figref{time2d-typing} illustrates using the typing rules of
\figref{type-terms} to perform progressive typing our four-line
motivating example~(\figref{full-example-code}).
%
The vertical and horizontal dimensions of the table list each of the
four lines; the vertical axis represents concrete execution, and the
horizontal axis represents typing the four right-hand-sides of the
program's four let-bindings, and in particular, for
\lstinline{filterDb} (on Line 2) and \lstinline{joinDb} (on Line 4),
the table indicates whether the operation was typed in the uncertain
or certain modality.
%
As execution progresses (vertically) over Lines 1 and 3, the
typing of the program continuation's becomes more certain: After Line
1 executes, Line 2 types in the certain modality ($[[!]]$) instead of
the uncertain modality ($[[?]]$); similarly, after Line 3, Lines 4
onward type using the certain modality.
%
As the final column shows, the certainty of code using these tables in
the remainder of the program (Line 5 onwards) increases after each of the two calls to
\lstinline{openDb}.  Between the two calls, some information is known
(relating to the first two tables defined on Lines 1 and 2), but some
information is still missing (relating to the two tables defined in Lines 3
and 4).

Our current Rust-based prototype of \lambdaVMF is powerful enough to
express this example, including the progressive typing discussed
above.
%\footnote{\url{https://github.com/cuplv/vmfuture} }
%
In \secref{discuss}, we discuss the potential to use incremental
computation in the context of such progressive typing; the goal is to
improve performance by exploiting the redundancy of re-typing the
program's continuation.




















\iffalse

\paragraph{Program syntax: CBPV.}
For economy of both implementation and reasoning, the syntax of VMF
programs is directly insipired by that of the Call-by-Push-Value
(CPBV) syntax and evaluation strategy~\cite{CBPV}.
%
CBPV is similar to CBV, except that unlike CBV, CBPV neatly separates
the concept of a thunked computation from that of a lambda
abstraction.
%
Like other administrative normal forms, CPBV also imposes a separation
of values and computations, in terms of syntax and semantics.
%
Computations that eliminate values have value sub-terms.
%
In contrast to computation forms, value forms consist of (passive,
non-doing) data types; specifically, here we consider variables
(ranging over previously-defined values), primitives (viz., numbers
and strings), records of values, store locations, open thunks that
suspend a computation term as a value~($[[othunk e]]$) and thunks
closed by an environment~($[[thunk env e]]$).

Unlike values, computations consist of program terms that actively
\emph{do things}, and for which the VM defines operational steps. For
instance, field projection from a record value is a computation, since
it eliminates a value (viz., the record that contains the projected
field) and introduces a new one.
%
Though CBV treats lambdas as values, the distinctive quirk of CBPV is
that function abstraction is a computation (not a value) and that it
interacts with function applications via an ambient stack (hence,
``call-by-\emph{push}-value''):
%
Function application~$[[e v]]$ uses a function abstraction by pushing
an argument value~$v$ on this ambient stack and then running the
function body~$e$.
%
Lambdas~$[[lam x.e]]$ abstract over a variable~$x$ by popping a value
for~$x$ from this ambient stack.
%
Compared with CBV, the presence of this ambient stack streamlines the
expression of currying.
%
Specifically, CBPV avoids the need for creating closures that
represent the partially-applied lambdas in the curried series.
%
Below, we will augment these (standard) computations and values with
computations over simple databases.

\begin{figure}
\small
\begin{mathpar}
\Infer{lam}
{[[Ctx, x : A |- e       : C]]}
{[[Ctx        |- lam x.e : A -> C]] }
\and
\Infer{app}
{[[Ctx |- e : A -> C]]
\\\\
[[Ctx |- v : A]]
}
{[[Ctx |- e v : C]]}
\and
\Infer{proj?}
{[[Ctx |- v1 : ?]]
\\\\
[[Ctx |- v2 : ?]]
}
{[[Ctx |- proj ? v1 v2 : F ?]] }
\and
\Infer{proj!}
{[[Ctx |- v1 : Dict (Delta, v2 => A)]]
\\\\
[[Ctx |- v2 : B]]
}
{[[Ctx |- proj ! v1 v2 : F A]] }
\and
\Infer{openDb?}
{[[Ctx |- v : Str]]}
{[[Ctx |- openDb ? v : F (Db ?)]]}
\and
\Infer{filterDb?}
{[[Ctx |- v1 : Db ?]]
\\
[[Ctx |- v2 : U(? -> F Bool)]]
}
{[[Ctx |- filterDb ? v1 v2 : F (Db ?)]]}
\and
\Infer{filterDb!}
{[[Ctx |- v1 : Db A]]
\\
[[Ctx |- v2 : U(A -> F Bool)]]
}
{[[Ctx |- filterDb ! v1 v2 : F (Db A)]]}
\and
\Infer{joinDb?}
{[[Ctx |- v1 : Db ?]]
\\
[[Ctx |- v2 : B2]]
\\\\
[[Ctx |- v3 : Db ?]]
\\
[[Ctx |- v4 : B4]]
}
{[[Ctx |- joinDb ? v1 v2 v3 v4 : F (Db ?)]]}
\and
\Infer{joinDb!}
{[[Ctx |- v1 : Db (Dict (Delta1, v2 => A))]]
\\
[[Ctx |- v2 : B2]]
\\
[[Ctx |- v3 : Db (Dict (Delta3, v4 => A))]]
\\
[[Ctx |- v4 : B4]]
}
{[[Ctx |- joinDb ! v1 v2 v3 v4 : F (Db (Dict (Delta1, v2 => A, Delta3, v4 => A)))]]}
\end{mathpar}
\caption{Selected typing rules}
\end{figure}

\fi

